Transformers in Action: Weakly Supervised Action Segmentation

The video action segmentation task is regularly explored under weaker forms of supervision, such as transcript supervision, where a list of actions is easier to obtain than dense frame-wise labels. In this formulation, the task presents various challenges for sequence modeling approaches due to the emphasis on action transition points, long sequence lengths, and frame contextualization, making the task well-posed for transformers. Given developments enabling transformers to scale linearly, we demonstrate through our architecture how they can be applied to improve action alignment accuracy over the equivalent RNN-based models with the attention mechanism focusing around salient action transition regions. Additionally, given the recent focus on inference-time transcript selection, we propose a supplemental transcript embedding approach to select transcripts more quickly at inference-time. Furthermore, we subsequently demonstrate how this approach can also improve the overall segmentation performance. Finally, we evaluate our proposed methods across the benchmark datasets to better understand the applicability of transformers and the importance of transcript selection on this video-driven weakly-supervised task.

==> tables/baselinesegmentation.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c|c}
        \hline
        Features           & \multicolumn{3}{c}{Action Segmentation F-acc.}                                            \\
        \hline
        \textbf{Breakfast} & NN-Vit. \cite{richard2018neuralnetwork}        & CDFL \cite{li2019weakly} & \textbf{Ours} \\
        \hline
        IDT                & \textbf{42.5}                                  & \textbf{49.9}            & \textbf{50.2} \\
        I3D                & 12.7                                           & 35.2                     & 45.1          \\
        SlowFast           & 18.5                                           & 35.8                     & 46.2          \\
        \hline
        \textbf{Hollywood} & NN-Vit. \cite{richard2018neuralnetwork}        & CDFL \cite{li2019weakly} & \textbf{Ours} \\
        \hline
        IDT                & \textbf{31.5}                                  & \textbf{45.1}            & \textbf{45.2} \\
        I3D                & 10.2                                           & 30.2                     & 41.2          \\
        SlowFast           & 14.4                                           & 31.6                     & 41.7          \\
        \hline
        \textbf{50 Salads} & NN-Vit. \cite{richard2018neuralnetwork}        & CDFL \cite{li2019weakly} & \textbf{Ours} \\
        \hline
        IDT                & \textbf{48.5}                                  & \textbf{54.1}            & \textbf{54.7} \\
        I3D                & 23.2                                           & 43.2                     & 53.8          \\
        SlowFast           & 25.9                                           & 45.6                     & 52.9          \\
        \hline
    \end{tabular}
    \caption{\textbf{Baseline Action Segmentation} - We first consider the implications of the modified GRU configurations on the existing inference pipeline. From this, we show how our method improves performance over existing pipelines, especially on network features.}\label{tab:baseline}
\end{table}

==> tables/combinedsegmentation.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c|c|c}
        \hline
        Method                          & Feat.                & T. Selector              & TSim           & F-acc.        \\
        \hline
        \multicolumn{5}{c}{\textbf{Breakfast}}                                                                             \\
        \hline
        CDFL \cite{li2019weakly}        & \multirow{4}{*}{IDT} & \multirow{3}{*}{Scoring} & -              & 50.2          \\
        \cline{1-1}

        DP-DTW \cite{chang2021learning} &                      &                          & -              & 50.8          \\
        \cline{1-1}

        \multirow{4}{*}{Ours}           &                      &                          & 0.694          & 50.1          \\
        \cline{3-3}
                                        &                      & \multirow{3}{*}{w/ Emb.} & 0.667          & 47.9          \\

        \cline{2-2}
                                        & I3D                  &                          & \textbf{0.712} & \textbf{51.2} \\
        \cline{2-2}
                                        & SlowF.               &                          & 0.679          & 49.6          \\
        \hline
        \multicolumn{5}{c}{\textbf{Hollywood Extended}}                                                                    \\
        \hline
        CDFL \cite{li2019weakly}        & \multirow{4}{*}{IDT} & \multirow{3}{*}{Scoring} & -              & 45.0          \\
        \cline{1-1}

        DP-DTW \cite{chang2021learning} &                      &                          & -              & \textbf{55.6} \\
        \cline{1-1}

        \multirow{4}{*}{Ours}           &                      &                          & 0.737          & 45.0          \\
        \cline{3-3}
                                        &                      & \multirow{3}{*}{w/ Emb.} & \textbf{0.740} & 45.7          \\

        \cline{2-2}
                                        & I3D                  &                          & 0.695          & 41.8          \\
        \cline{2-2}
                                        & SlowF.               &                          & 0.721          & 43.7          \\
        \hline
        \multicolumn{5}{c}{\textbf{50 Salads}}                                                                             \\
        \hline
        CDFL \cite{li2019weakly}        & \multirow{4}{*}{IDT} & \multirow{3}{*}{Scoring} & -              & \textbf{54.7} \\
        \cline{1-1}

        DP-DTW \cite{chang2021learning} &                      &                          & -              & -             \\
        \cline{1-1}

        \multirow{4}{*}{Ours}           &                      &                          & \textbf{0.584} & 54.5          \\
        \cline{3-3}
                                        &                      & \multirow{3}{*}{w/ Emb.} & 0.472          & 45.3          \\

        \cline{2-2}
                                        & I3D                  &                          & 0.553          & 49.9          \\
        \cline{2-2}
                                        & SlowF.               &                          & 0.558          & 50.3          \\
        \hline
    \end{tabular}
    \caption{\textbf{Action Segmentation (Combined)} - We compare the performance of our combined approach (using a single feature type) to reported results from existing works.}\label{tab:combined}
\end{table}

==> tables/embedding.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c|c|c}
        \hline
        \multirow{3}{*}{Dataset} & \multicolumn{4}{c}{TSim}                                                          \\
        \cline{2-5}
                                 & \multicolumn{3}{c|}{$k=1$ Embedding} & Scoring                                    \\
        \cline{2-5}
                                 & IDT                                  & I3D            & SlowFast & IDT            \\
        \hline
        \textbf{Breakfast}       & 0.65                                 & \textbf{0.739} & 0.714    & 0.694          \\
        \textbf{Hollywood}       & 0.732                                & 0.691          & 0.707    & \textbf{0.738} \\
        \textbf{50 Salads}       & 0.463                                & 0.561          & 0.568    & \textbf{0.584} \\
        \hline
    \end{tabular}
    \caption{\textbf{Transcript Embedding Performance} - Focusing on the transcript selection task with various features, we compare the suitability of transcripts taken from the embedding (single nearest neighbor) to those from the brute-force scoring method.}\label{tab:transcript}
\end{table}

==> tables/embeddingsegmentation.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c|c|c}
        \hline
        Dataset                             & Selector                 & $k$ & F-acc.        & Runtime        \\
        \hline
        \multirow{5}{*}{\textbf{Breakfast}} & Scoring                  & 237 & 50.2          & 31:24          \\
        \cline{2-3}
                                            & \multirow{4}{*}{w/ Emb.} & 1   & 51.5          & \textbf{00:17} \\
                                            &                          & 10  & 52.2          & 01:29          \\
                                            &                          & 50  & \textbf{53.1} & 03:11          \\
                                            &                          & 100 & 53.0          & 08:57          \\
        \hline
        \multirow{5}{*}{\textbf{Hollywood}} & Scoring                  & 361 & 43.4          & 02:37          \\
        \cline{2-3}
                                            & \multirow{4}{*}{w/ Emb.} & 1   & 40.0          & \textbf{00:03} \\
                                            &                          & 10  & 42.6          & 00:04          \\
                                            &                          & 50  & \textbf{46.0} & 00:07          \\
                                            &                          & 100 & 45.7          & 00:10          \\
        \hline
        \multirow{4}{*}{\textbf{50 Salads}} & Scoring                  & 40  & \textbf{54.7} & 35:43          \\
        \cline{2-3}
                                            & \multirow{3}{*}{w/ Emb.} & 1   & 40.7          & \textbf{00:50} \\
                                            &                          & 10  & 47.8          & 04:00          \\
                                            &                          & 25  & 50.1          & 20:47          \\
        \hline
    \end{tabular}
    \caption{\textbf{Transcript Embedding with Action Segmentation} - We consider how using a separately-trained embedding (using the best performing features) can affect the inference time segmentation performance and runtime (mm:ss), specifically when more nearest neighbors ($k$) are used.}\label{tab:segembed}
\end{table}

==> tables/features.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c}
        \hline
        Name                                      & Type                             & Frame Dimension \\
        \hline
        IDT \cite{wang2013action}                 & Handcrafted                      & 64              \\
        \cline{2-2}
        I3D \cite{carreira2017quo}                & \multirow{2}{*}{Network-Derived} & 2048            \\
        SlowFast \cite{feichtenhofer2019slowfast} &                                  & 2304            \\
        \hline
    \end{tabular}
    \caption{\textbf{Types of Features} - In addition to the handcrafted IDT features from past approaches, we additionally utilize network features, including I3D as in MuCon \cite{souri2021fast}, as well as from the newer SlowFast architecture.}\label{tab:features}
\end{table}
